Galaxy evolution through infrared and submillimeter spectroscopy: Measuring star formation and black hole accretion with JWST and ALMA

Rest-frame mid- to far-infrared spectroscopy is a powerful tool to study how galaxies formed and evolved, because a major part of their evolution occurs in heavily dust enshrouded environments, especially at the so-called Cosmic Noon. Using the calibrations of IR lines we predict the expected fluxes of lines and features, with the aim to measure the star formation rate and the Black Hole Accretion rate in intermediate to high redshift galaxies. The launch of the James Webb Space Telescope will allow us a deep investigation of both the SF and the BHA obscured processes as a function of cosmic time. We assess the spectral lines and features that can be detected by JWST-MIRI in galaxies and Active Galactic Nuclei up to redshift z= 3. We confirm the fine-structure lines of [MgIV]4.49um and [ArVI]4.53um as good BHA rate tracers for the 1<z<3 range, and we propose the [NeVI]7.65um line as the best tracer for redshifts of z<1.5. We suggest the use of the [ArII]6.98um and [ArIII]8.99um lines to measure the SF rate, for z<3 and z<2. At higher redshifts, the PAH features at 6.2um and 7.7um can be observed at z<3 and z<2.7 respectively. Rest-frame far-IR spectroscopy is currently being collected in high redshift galaxies (z>3) with the Atacama Large Millimeter Array. We confirm that the [CII]158um line is a good tracer of the SF rate and can in most cases (0.9<z<2 and 3<z<9) be observed, and we propose the use of the combination of [OIII]88um and [OI]145um lines as an alternative SF rate tracer, that can be detected above z>3. We conclude, however, that the current and foreseen facilities will not be able to cover properly the peak of the obscured SF and BHA activities at the Cosmic Noon of galaxy evolution and a new IR space telescope, actively cooled to obtain very good sensitivities, covering the full IR spectral range from about 10um to 300um, will be needed.

==> immagini/jwst_alma_sim.tex <==
\begin{abstract}
Rest-frame mid- to far-infrared (IR) spectroscopy is a powerful tool to study how galaxies formed and evolved, because a major part of their evolution occurs in heavily dust enshrouded environments, especially at the so-called Cosmic Noon (i.e. at 1$<$z$<$3). 
Using the calibrations of IR lines, recently updated with {\it Herschel} and {\it Spitzer} spectroscopy, we predict the expected fluxes of lines and features, with the aim to measure the star formation (SF) rate and the Black Hole Accretion (BHA) rate in intermediate to high redshift galaxies.

On the one hand, the launch of the James Webb Space Telescope (JWST) in a short time, together with its mid-IR spectroscopic capability, will allow us for the first time a deep investigation of both the SF and the BHA obscured processes as a function of cosmic time. We make an assessment of the spectral lines and features that can be detected by JWST-MIRI in galaxies and Active Galactic Nuclei up to redshift $z \sim 3$. We confirm the fine-structure lines of [MgIV]4.49$\mu$m and [ArVI]4.53$\mu$m as good BHA rate tracers for the 1$\lesssim$ z$\lesssim$3 range, and we propose the [NeVI]7.65$\mu$m line as the best tracer for redshifts of z$\lesssim$1.5. We suggest the use of the [ArII]6.98$\mu$m and [ArIII]8.99$\mu$m lines to measure the SF rate, for z$\lesssim$3 and z$\lesssim$2, respectively, while the stronger [NeII]12.8$\mu$m exits the JWST-MIRI spectral range above z$\gtrsim$ 1.2. At higher redshifts, the PAH features at 6.2$\mu$m and 7.7$\mu$m can be observed at z$\lesssim$3 and z$\lesssim$2.7, respectively.

On the other hand, rest-frame far-IR spectroscopy is currently being collected in high redshift galaxies (z$\gtrsim$3) since a few years with the Atacama Large Millimeter Array (ALMA). The observability of far-IR lines from ALMA depends on the frequency at which the line is redshifted, the higher the frequency the most difficult is observing the line, because of the decrease of atmospheric transmission.
While the [CII]158$\mu$m line, a good tracer of the SF rate, can in most cases (0.9$\lesssim$z$\lesssim$2 and 3$\lesssim$z$\lesssim$9) be observed, the other far-IR lines from oxygen and nitrogen can hardly be detected in discrete redshift ranges, and their predicted detection in high-z galaxies strongly depends on their assumed metallicity.

We conclude, however, that the current and foreseen facilities will not be able to cover properly the peak of the obscured SF and BHA activities at the Cosmic Noon of galaxy evolution and a new IR space telescope, actively cooled to obtain very good sensitivities, covering the full IR spectral range from about 10$\mu$m to 300$\mu$m, will be needed.
\end{abstract}

\section{INTRODUCTION}
\label{sec:intro}
The investigation on how galaxies form and evolve is one of the main fields of study of modern astrophysics, and it is significantly hindered by the limited knowledge concerning the main processes that participate in this evolution. From an observational point of view, the evolution is energetically dominated by two processes, namely star formation, with the subsequent stellar evolution, and the accretion onto the supermassive black holes in galactic nuclei. The bulk of activity, however, takes place at the so-called \emph{Cosmic Noon} (z$\sim$1-3) in heavily dust obscured environments, where almost 90$\%$ of optical and UV radiation is absorbed by dust and re-emitted at longer wavelengths \citep{madau2014,heckman2014}, then followed by a steep decline toward the present epoch. Thus, to fully characterize the various phenomena driving galaxy evolution and their interplay is paramount to explore galaxies throughout their dust obscured phase \citep[e.g.][]{spinoglio2017,spinoglio2021}.

The mid- to far-infrared (IR) spectral range is populated by a wealth of lines and features which offer an ideal tool to probe the dust  hidden regions where the bulk of activity takes place \citep[e.g.][]{spinoglio1992,armus2007}. The various fine-structure lines in this range cover a wide range of physical parameters such as density, ionization and excitation, and can be used to discriminate between the different conditions of the interstellar medium and the processes taking place there. Most of these lines, however, can be observed only from space IR telescopes, while only a limited number of transitions are detectable by ground-based facilities. In particular, AGN activity can be traced by high-ionization lines, while low to intermediate ionization fine-structure lines are good tracers of star formation processes.

\begin{figure*}
    \centering
    \includegraphics[width=0.5\textwidth]{immagini/miri_range.pdf}~
    \includegraphics[width=0.5\textwidth]{immagini/alma_range.pdf}
    \caption{\textit{Left:} observability of key mid-IR (dashed lines) lines as a function of redshift. The shaded area shows the redshift interval covered by the \textit{JWST}-MIRI instrument spectral range. \textit{Right:} observability of key far-IR (dashed lines) lines compared to the ALMA bands (shaded area) in the 1-8 redshift interval. Dots represent current detection for each line. Figure adapted from \citet{mordini2021}.}
    \label{fig:miri_alma_spectral_range}
\end{figure*}

The \emph{James Webb Space Telescope} \citep[JWST,][]{gardner2006}, due to be launched in December 2021, will observe the Universe in the near- to mid-IR range. In particular, the Mid-InfraRed Instrument \citep[MIRI, ][]{rieke2015,wright2015} will be able to obtain imaging and spectra with unprecedented sensitivity in the 4.9–28.9$\mu$m range. In a near future the extremely large ground-based telescopes under construction, with dedicated instruments for N-band spectroscopy, will be able to obtain observations in the mid-IR atmospheric windows at 8–13$\mu$m and thus measure the fine structure lines of [SIV]10.5$\mu$m and [NeII]12.8$\mu$m, and the PAH at 11.3$\mu$m in local galaxies. The ESO Extremely Large telescope \citep[E-ELT;][]{gilmozzi2007} is expected to obtain first light at the end of 2025, with the Mid-infrared ELT Imager and Spectrograph \citep[METIS;][]{brandl2021} covering the N band with imaging and low resolution spectroscopy; the Thirty Meter Telescope \citep[TMT;][]{schock2009} will have completed first light and will be ready for science at the end of 2027, and the Giant Magellan Telescope \citep[GMT;][]{johns2012} will be operational in 2029.

At the present time, only the \emph{Stratospheric Observatory For Infrared Astronomy} \citep[SOFIA;][]{gehrz2009}, observing from the high atmosphere, can cover the full mid- to far-IR spectral range and detect emission for the brightest galaxies in the local Universe, although with limitations from atmospheric absorption and emission. 

At much longer wavelengths, in the submillimeter domain, the \emph{Atacama Large Millimeter Array} \citep[ALMA; ][]{wootten2009} can observe within the submillimeter atmospheric bands centered at $\sim$ 350, 450, 700 and  950$\mu$m. However the shorter wavelengths bands are accessible only when the precipitable water vapour content of the atmosphere is very low (PWV $\lesssim$0.5 mm) to obtain a peak transmission over 50\%.

In this paper, we assess the detection of star formation and BHA tracers using the JWST-MIRI spectrometer and the ALMA telescope, by computing the predicted fluxes of key lines as a function of redshift and comparing them with the sensitivity of the two instruments. The work is organized as follows: Sections \ref{sec:jwst} and \ref{sec:alma} briefly describe the capabilities of the JWST-MIRI instrument and the ALMA observatory, respectively, for studying galaxy evolution.
Section \ref{sec:methods} describes the approach used to derive the predicted flux of the lines, Section \ref{sec:results} reports our results, and in particular the predictions concerning JWST in Section \ref{sec:results_jwst} and ALMA in Section \ref{sec:results_alma}; in Section \ref{sec:discussion} we discuss our results, while our conclusions are presented in Section \ref{sec:conclusions}.

\subsection{The Cosmic Noon as seen by JWST in the mid-IR}
\label{sec:jwst}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.95\textwidth]{immagini/alma_range.pdf}
%    \caption{Observability of key far-IR (dashed lines) lines compared to the ALMA bands (shaded area) in the 1-8 redshift interval. Dots represent current detection for each line.}
%    \label{fig:alma_spectral_range}
%\end{figure}

\begin{table}[t]
\caption{The fine-structure lines in the mid- to far-IR range used in this work. For each line, the columns give: central wavelength, frequency, ionization potential, excitation temperature and critical density. Critical densities and excitation temperatures are from: \citet{launay1977,tielens1985,greenhouse1993,sturm2002,cormier2012,goldsmith2012,farrah2013,satyapal2021}. Adapted from \citet{mordini2021}.}
\label{tab:line_properties}
\begin{tabular}{lccccc}
\bf Line & \bf $\lambda$ & \bf $\nu$ & \bf I.P. & \bf E & \bf $n_{\rm cr}$ \\
 & ($\, \mu$m) & (GHz) & (eV) & (K) & ($\rm{cm^{-3}}$) \\ \hline
$[\rm{MgIV}]$ & 4.49 & 66811.78& 80 &--& 1.258$\times$10$^{7}$ \\
$[\rm{ArVI}]$ & 4.53 & 66208.58& 75 &-- & 7.621$\times$10$^{5}$ \\
$[\rm{ArII}]$ & 6.98 &42929.48& 16 &-- & 4.192$\times$10$^{5}$ \\
$[\rm{NeVI}]$ & 7.65 & 39188.56 & 126.21 & 1888 & $2.5 \times 10^5$ \\
$[\rm{ArIII}]$ & 8.99 & 33351.11& 28 & -- & 3.491$\times$10$^{5}$ \\
$[\rm{SIV}]$ & 10.51 & 28524.50 & 34.79 & 1369 & $5.39 \times 10^4$ \\
$[\rm{NeII}]$ & 12.81 & 23403.00 & 21.56 & 1123 & $7.00 \times 10^5$ \\
$[\rm{NeV}]$ & 14.32 & 20935.23 & 97.12 & 1892 & $3 \times 10^4$ \\
$[\rm{OI}]$ & 63.18 & 4744.77 & -- & 228 & $4.7 \times 10^5$\tnote{a} \\
$[\rm{OIII}]$ & 88.36 & 3393.01 & 35.12 & 163 & $510$ \\
$[\rm{NII}]$ & 121.90 & 2459.38 & 14.53 & 118 & $310$ \\
$[\rm{OI}]$ & 145.52 & 2060.07 & -- & 98 & $9.5 \times 10^4$\tnote{a} \\
$[\rm{CII}]$ & 157.74 & 1900.54 & 11.26 & 91 & $20$,$[2.2\tnote{a},4.4\tnote{b}\ ]\times 10^3$ \\
$[\rm{NII}]$ & 205.3 & 1460.27 & 14.53 & 70 & $48$\\
 \hline
\end{tabular}%
\begin{tablenotes}
    \item[a] Critical density for collisions with hydrogen atoms.
    \item[b] Critical density for collisions with H$_2$ molecules.
\end{tablenotes}
\end{table}

The JWST-MIRI instrument can perform spectroscopic imaging observations in the 4.9–28.9 $\mu$m range through integral field units. The left panel in Fig. \ref{fig:miri_alma_spectral_range} shows the instrument spectral range and the maximum redshift at which key lines and features in the mid-IR range can be observed. The JWST-MIRI cut-off wavelength of $\sim$29$\mu$m  significantly limits the possibility of probing accretion phenomena through the brightest lines, unobservable beyond redshift z>1, missing about half of the accretion history. The best spectroscopic tracers to measure the BHAR in the mid-IR, i.e. [\ion{Ne}{v}]$14.3,24.3\, \rm{\micron}$ and [\ion{O}{iv}]$25.9\, \rm{\micron}$, cannot be observed beyond the local Universe, $z \gtrsim 0.9$ in the best case \citep[see, e.g.][]{sturm2002,melendez2008,tommasin2008,tommasin2010}. The [NeV]24.3 $\mu$m and [OIV]25.9 $\mu$m lines are not shown in the left panel of Fig. \ref{fig:miri_alma_spectral_range} due to the limited range available: the former line can be observed up to redshift z$\simeq$0.15, and the latter line can be observed up to redshift z$\simeq$0.1. The [NeV]14.3 $\mu$m line can be observed by JWST-MIRI up to redshift z$\simeq$1. 

Alternative tracers for BHAR that could be used with the JWST-MIRI to probe the accretion processes beyond redshift z$\sim$1 have been proposed by \citet{satyapal2021}: these authors analyze the possibility of detecting Compton-thick AGNs using an integrated modeling approach in which both the line and emergent continuum are predicted from gas exposed to the ionizing radiation from a young starburst or an AGN, focusing specifically on the spectral diagnostics available through the instruments MIRI and NIRSpec \citep[Near Infrared Spectrograph;][]{bagnasco2007,birkmann2016}. In particular, they provide predictions of the detectability of key diagnostic lines such as [MgIV]4.49 $\mu$m, [ArVI]4.53$\mu$m and [NeVI]7.65$\mu$m, which appear to be ideal tracers of heavily obscured AGN and can potentially be detected in AGN with moderate activity up to redshift z$\sim$3. These lines, however, have not been extensively observed so far, and their behaviour is mainly derived from photo-ionization models.

At the same time, star forming galaxies up to redshift z$\sim$2 could be traced only by the PAH features, which behaviour at high redshifts is not yet well understood.  These features could in fact be destroyed by a strong radiation field, or be less efficiently formed due to low metallicity, \citep[e.g. ][]{engelbracht2008,cormier2015,galliano2021}. On the other hand, while alternative SFR tracers can be found in optical lines \citep[e.g.][]{alvarezmarquez2019} or photometric bands \citep[e.g.][]{senarath2018}, mid-IR spectroscopic tracers have not yet been analyzed.
\subsection{Galaxy evolution with ALMA beyond the Cosmic Noon}
\label{sec:alma}

While the JWST will allow us to probe galaxies at redshift below z$\lesssim$3 using mid-IR lines, the ALMA telescope will allow us to probe galaxies at redshifts z$\gtrsim$3. In particular, the SFR could be traced using far-IR lines, like the [OIII]88$\mu$m and the [CII]158$\mu$m lines up to redshift z$\simeq$8, as shown in the right panel of Fig. \ref{fig:miri_alma_spectral_range}, providing important information on the evolution of galaxies with cosmic time. An analogous figure can be found in \citet[][see their fig.\,1]{carilli2013}, where the CO transitions and other key tracers of the ISM are shown as a function of redshift versus frequency in terms of the observability by ALMA and JVLA \citep[Karl J. Jansky Very Large Array,][]{perley2011}. As can be seen in the right panel of Fig. \ref{fig:miri_alma_spectral_range}, the [OIII]88$\mu$m, [CII]158$\mu$m and [NII]205$\mu$m lines have been detected over an extended redshift interval, from z$\sim$3-4 to z$\sim$6-8, while the shorter wavelength lines, such as [OI]63$\mu$m, present very few results. No detections have been reported so far for the [OIII]52$\mu$m and [NIII]57$\mu$m lines. This is due to the difficulty of observing in the bands at higher frequency, for which the atmospheric absorption allows good visibility only for $\sim$10$\%$ of the total observational time. While ALMA cannot detect these far-IR fine-structure lines in galaxies at the peak of their activity (1$\lesssim$z$\lesssim$3), it allows us to probe galaxies at earlier epochs, thus shedding light on what processes led to the cosmic noon. The observations  available in the rest-frame far-IR continuum, due to thermal emission, suggest that, even before the cosmic noon, dust was already present in galaxies active regions \citep[e.g.][]{laporte2017}, and IR tracers are needed in order to probe these obscured regions and understand the physical processes taking place.

\begin{table}[t]
\caption{Line ratios derived from CLOUDY simulations by \citet{fernandez2016} for AGN, SFG and LMG: log(U) indicates the logarithm of the ionization parameter, while log(n$_{H}$) indicates the logarithm of the hydrogen density.}
\label{tab:line_ratios}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lc|cccc}
\hline
AGN & \multicolumn{1}{r|}{log(U)} & -1.5 & -1.5 & -2.5 & -2.5 \\
 & \multicolumn{1}{r|}{log(n$_{H}$)} & 2 & 4 & 2 & 4 \\[0.1cm] \cline{3-6} 
 & {[MgIV]}4.49/[NeV]14.3 & 0.09 & 0.11 & 0.72 & 1.00 \\
 & {[ArVI]}4.53/[NeV]14.3 & 0.10 & 0.14 & 0.03 & 0.04 \\
 & {[NeVI]}7.68/[NeV]14.3 & 0.58 & 0.78 & 0.04 & 0.06 \\[0.15cm] \cline{3-6} 
SFG & \multicolumn{1}{r|}{log(U)} & -2.5 & -2.5 & -3.5 & -3.5 \\
 & \multicolumn{1}{r|}{log(n$_{H}$)} & 1 & 3 & 1 & 3 \\[0.1cm] \cline{3-6} 
 & {[ArII]}6.98/[NeII]12.8 & 0.05 & 0.06 & 0.12 & 0.12 \\
 & {[ArIII]}8.99/[NeII]12.8 & 0.66 & 0.68 & 0.32 & 0.32 \\
 & $\frac{\rm [ArII]6.98 + [ArIII]8.99}{\rm [NeII]12.8 + [NeIII]15.6}$ & 0.30 & 0.30 & 0.38 & 0.38 \\[0.15cm] \cline{3-6} 
LMG & \multicolumn{1}{r|}{log(U)} & -2 & -2 & -3 & -3 \\
 & \multicolumn{1}{r|}{log(n$_{H}$)} & 1 & 3 & 1 & 3 \\[0.1cm] \cline{3-6} 
 & {[ArII]}6.98/[NeII]12.8 & 0.12 & 0.12 & 0.12 & 0.11 \\
 & {[ArIII]}8.99/[NeII]12.8 & 8.31 & 8.29 & 1.41 & 1.40 \\
 & $\frac{\rm [ArII]6.98 + [ArIII]8.99}{\rm [NeII]12.8 + [NeIII]15.6}$ & 0.19 & 0.18 & 0.27 & 0.27 \\[0.15cm]
\hline
\end{tabular}%
}
\end{table}


\section{METHODS}
\label{sec:methods}

We assess how the JWST-MIRI and ALMA instruments can measure the star formation rate (SFR) and the black hole accretion rate (BHAR) covering, respectively, the z$\lesssim$3 and z$\gtrsim$3 redshift intervals. The predictions for JWST-MIRI have been derived using the CLOUDY \citep{ferland2017} photo-ionization models computed by \citet{fernandez2016}, using the BPASS v2.2 stellar population synthetic library \citep{stanway2018} for the case of the star forming models. We consider, in particular, three classes of objects, as presented in \citet{mordini2021}: \textit{i)} AGN, \textit{ii)} star forming galaxies (SFG), and \textit{iii)} low metallicity galaxies (LMG) covering the $\sim$7$\leq$12 + log (O/H)$\leq$8.5 metallicity range \citep{madden2013,cormier2015}. This is motivated by the detection of massive galaxies ($\sim$10$^{10}$ M$_{\odot}$) in optical surveys with sub-solar metallicities during the cosmic noon, which may experience a fast chemical evolution above z$\sim$2 \citep{maiolino2008,mannucci2009,troncoso2014,onodera2016}. These changes are expected to have an impact on the ISM structure of high-z galaxies, favouring stronger radiation fields \citep[e.g.][]{steidel2016,kashino2019,sanders2020} and a more porous ISM similar to that observed in dwarf galaxies \citep{cormier2019}.

To measure the BHAR, we consider the [MgIV] 4.49$\mu$m, [ArVI] 4.53$\mu$m \citep[see, e.g.,][]{satyapal2021} and the  [NeVI] 7.65$\mu$m line. 
We need to caution the reader about the use of the [NeVI]7.65$\mu$m line, because its detections by the Infrared Space Observatory (ISO) \citep{sturm2002}, on which is based the calibration \citep{mordini2021} are scarce and have only been obtained for the brightest sources, and therefore this calibration is uncertain.
The [ArII]6.98$\mu$m and [ArIII]8.99$\mu$m lines are suitable to measure the SFR. The properties of these lines are summarized in Table \ref{tab:line_properties}.  

For the BHAR tracers, we use the template of an AGN of total IR luminosity of  L$_{IR}$=10$^{12}$L$_{\odot}$, to represent the bulk of the population at redshift z$\sim$2. We use four different photo-ionization models to derive the line intensities, with two values of the ionization parameter: log\,$U$=-1.5 and log\,$U$=-2.5, and two values of the hydrogen density: log(n$_{H}$/cm$^{-3}$)=2 and log(n$_{H}$/cm$^{-3}$)=4. The calibration of the line luminosities, against the total IR luminosities, has been derived using the ratios of the high-excitation magnesium, argon and neon lines relative to the [NeV]14.3$\mu$m line in the photo-ionization models, and the calibration of the [NeV]14.3$\mu$m line from \citet{mordini2021}.

For the SFR tracers, we consider both SFG and LMG, deriving, in both cases, the line intensities dependent on the calibration of the [NeII]12.8$\mu$m line \citep{mordini2021} considering, for the SFG, photo-ionization models with an ionization parameter of log\,$U$=-2.5 and log\,$U$=-3.5, and a hydrogen density of log(n$_{H}$/cm$^{-3}$)=1 and log(n$_{H}$/cm$^{-3}$)=3, for a total of four different cases. For the LMG we consider an ionization parameter of log\,$U$=-2 and log\,$U$=-3, and hydrogen densities of log(n$_{H}$/cm$^{-3}$)=1 and log(n$_{H}$/cm$^{-3}$)=3. In both cases, we assume a total IR luminosity of the galaxy of L$_{IR}$=10$^{12}$L$_{\odot}$.

The predictions for the ALMA telescope were derived from the line calibrations described in \citet{mordini2021}. While the spectral range covered by ALMA has no unambiguous high ionization line that can be used to trace the BHAR, we explore what lines, or combination of them, can be used to trace the SFR.
Following \citet{mordini2021}, we consider the [CII]158$\mu$m line and the sum of two oxygen lines, either the [OI]63$\mu$m and [OIII]88$\mu$m, or the [OI]145$\mu$m and [OIII]88$\mu$m.



Table \ref{tab:line_properties} gives the key properties of the lines used in this work. Table \ref{tab:line_ratios} reports the line ratios used to derive the line intensities for the [MgIV]4.49$\mu$m, [ArVI]4.53$\mu$m, [ArII]6.98$\mu$m, [NeVI]7.65$\mu$m and [ArIII]8.99$\mu$m lines, given the different combinations of ionization parameter and hydrogen densities. Table \ref{tab:derived_correlations} reports the calibrations computed from the photo-ionization models scaled to the [NeII]12.8 $\mu$m and [NeV]14.3$\mu$m lines (see Section \ref{sec:results_jwst}), while the calibrations of the different lines and features in the mid- to far-IR range can be found in Table D.1 in \citet{mordini2021}.


\section{RESULTS}
\label{sec:results}

\subsection{Predictions for JWST}
\label{sec:results_jwst}

\begin{table}
\caption{Derived calibrations for the fine structure lines according to line ratios reported in Table \ref{tab:line_ratios}. For the AGN lines,the log\,$U$=-2.5 log(n$_{H}$/cm$^{-3}$)=2 values were used, log\,$U$=-3.5 log(n$_{H}$/cm$^{-3}$)=3 for the SFG and log\,$U$=-2 log(n$_{H}$/cm$^{-3}$)=1 for LMG.}
\label{tab:derived_correlations}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc}
\hline
\bf Line/feature & \bf AGN &  & \bf SFG &  & \bf LMG &  \\
 & $a$ & $b$ & $a$ & $b$  & $a$  & $b$  \\ \hline
{[MgIV]}4.49 & 1.32 & -5.15 & -- & -- & -- & -- \\
{[ArVI]}4.53 & 1.32 & -6.53 & -- & -- & -- & -- \\
{[NeVI]}7.65 & 1.32 & -6.41 & -- & -- & -- & -- \\
{[ArII]}6.98 & -- & -- & 1.04 & -4.4 & 1.37 & -5.28 \\
{[ArIII]}7.99 & -- & -- & 1.04 & -3.97 & 1.37 & -3.44
\end{tabular}%
}
\end{table}
 
In this section, we predict the intensities of the mid-IR lines and features in the 5-9$\mu$m range, as derived from CLOUDY models, and compare them with the JWST-MIRI sensitivity, to verify if these lines, used as tracers for SFR and BHAR, can be observed in objects at redshifts z$>$1. Table \ref{tab:derived_correlations} reports the derived correlations of the lines used in this work for the most common values of ionization potential (log\,$U$) and gas density [log(n$_{H}$/cm$^{-3}$)] for each type of object. For the AGN lines, we use the calibration of the [NeV]14.3$\mu$m line, while for SFG and LMG we use the [NeII]12.8$\mu$m line. Since these correlations are derived from CLOUDY simulations, we do not report the error on the coefficients. Fig.\,\ref{fig:miri_z1} shows the sensitivity of JWST-MIRI, highlighting the wavelengths at which the various fine-structure lines and PAH spectral features can be observed in a galaxy at redshift z=1. In the $\sim 5-16\mu$m rest-frame interval, the MIRI sensitivity is below $\sim$2$\times$10$^{-20}$W\,m$^{-2}$ for a 1hr, 5$\sigma$ observation, while in the $\sim 16-29\mu$m rest-frame wavelength interval, instead, the sensitivity is increasingly worse, going from $\sim$6$\times$10$^{-20}$W\,m$^{-2}$ at $\sim$16$\mu$m, to $\sim$10$^{-18}$W\,m$^{-2}$ at $\sim$29$\mu$m. This makes observing the [SIV]10.5$\mu$m, [NeII]12.8$\mu$m and [NeV]14.3$\mu$m lines a challenging task, and rises the need to find and analyze new possible tracers.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{immagini/miri_z1.png}
    \caption{Sensitivity of the JWST-MIRI instrument at different wavelengths, for a 1 hr., 5$\sigma$ observation. The symbols show the position, in the MIRI wavelength range, at which the different lines are observed in a galaxy at redshift z = 1. From left to right, the considered lines and feature, at their rest frame wavelength, are: [MgIV]4.49$\mu$m, [ArVI]4.53$\mu$m, PAH feature at 6.2$\mu$m, [ArII]6.98$\mu$m, [NeVI]7.65$\mu$m, PAH feature at 7.7$\mu$m, [ArIII]8.99$\mu$m, [SIV]10.5$\mu$m, [NeII]12.8$\mu$m and [NeV]14.3$\mu$m.}
    \label{fig:miri_z1}
\end{figure}


In the 5-16$\mu$m interval range, possible tracers for AGN activity are given by the [MgIV]4.49$\mu$m, [ArVI]4.53$\mu$m and [NeVI]7.65$\mu$m lines, while the [ArII]6.98$\mu$m and the [ArIII] 8.99$\mu$m lines can be used as tracers for star formation activity, together with the PAH feature at 6.2$\mu$m. Given their relatively short wavelength, these lines can be used to probe the highly obscured galaxies at the Cosmic Noon (1$\lesssim$z$\lesssim$3). 

\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{immagini/ne5_agn_miri_range.pdf}~
    \includegraphics[width=0.45\textwidth]{immagini/ar6_agn_miri_range.pdf}
    \includegraphics[width=0.45\textwidth]{immagini/mg4_agn_miri_range.pdf}~
    \includegraphics[width=0.45\textwidth]{immagini/ne6_agn_miri_range.pdf}
    \caption{Predicted fluxes, as a function of redshift, for an AGN with a  total IR luminosity of L$_{IR}$=10$^{12}$L$_{\odot}$ for the [NeV]14.3$\mu$m  (a:top left, red solid line); the [ArVI]4.5$\mu$m line (b:top right); the [MgIV]4.49$\mu$m line {\bf (c:bottom left)} and  for the [NeVI]7.65$\mu$m line (d: bottom right). In all figures, the black solid line shows the 1 hr., 5 $\sigma$ sensitivity of JWST-MIRI, while the grey dashed line shows the 1 hr., 5 $\sigma$ sensitivity of the SPICA SMI-LR \citep{kaneda2017}. In panels b, c and d, the red dash-dotted line shows the predicted flux for a galaxy with an ionization parameter of log\,$U$=-1.5 and a hydrogen density of log(n$_{H}$/cm$^{-3}$)=2, the blue dotted line indicates log\,$U$=-1.5 and log(n$_{H}$/cm$^{-3}$)=4, the green solid line shows log\,$U$=-2.5 and log(n$_{H}$/cm$^{-3}$)=2, and the pink dashed line shows log\,$U$=-2.5 and log(n$_{H}$/cm$^{-3}$)=4.}
    \label{fig:miri_ar6_mg4_ne6}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{immagini/ne2_sf_miri_range.pdf}~
    \includegraphics[width=0.45\textwidth]{immagini/ar2_sf_miri_range.pdf}
    \includegraphics[width=0.45\textwidth]{immagini/ar3_sf_miri_range.pdf}
    \caption{Predicted fluxes, as a function of redshift, of a SFG with a total IR luminosity of L$_{IR}$=10$^{12}$L$_{\odot}$ for the [NeII]12.8$\mu$m  (a:top left, red solid line); [ArII]6.98$\mu$m line (b:top right) and for the [ArIII]8.99$\mu$m line (c: bottom). In all figures, the black solid line shows the 1 hr., 5 $\sigma$ sensitivity of JWST-MIRI, while the grey dashed line shows the 1 hr., 5 $\sigma$ sensitivity of the SPICA SMI-LR \citep{kaneda2017}. In panels b and c, the red dash-dotted line shows a galaxy with an ionization parameter of log\,$U$=-2.5 and a hydrogen density of log(n$_{H}$/cm$^{-3}$)=1, the blue dotted line indicates log\,$U$=-2.5 and log(n$_{H}$/cm$^{-3}$)=3, the green solid line shows log\,$U$=-3.5 and log(n$_{H}$/cm$^{-3}$)=1, and the pink dashed line shows log\,$U$=-3.5 and log(n$_{H}$/cm$^{-3}$)=3.}
    \label{fig:miri_ar2_ar3_sf}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{immagini/ne2_lmg_miri_range.pdf}~
    \includegraphics[width=0.45\textwidth]{immagini/ar2_lmg_miri_range.pdf}
    \includegraphics[width=0.45\textwidth]{immagini/ar3_lmg_miri_range.pdf}
    \caption{Predicted fluxes, as a function of redshift, of a LMG with a total IR luminosity of L$_{IR}$=10$^{12}$L$_{\odot}$ for the [NeII]12.8$\mu$m (a:top left, red solid line); the [ArII]6.98$\mu$m line (b:top right) and the [ArIII]8.99$\mu$m line (c: bottom). In all figures, the black solid line shows the 1 hr., 5 $\sigma$ sensitivity of JWST-MIRI, while the grey dashed line shows the 1 hr., 5 $\sigma$ sensitivity of the SPICA SMI-LR \citep{kaneda2017}. In panels b and c, the red dash-dotted line shows a galaxy with an ionization parameter of log\,$U$=-2 and a hydrogen density of log(n$_{H}$/cm$^{-3}$)=1, the blue dotted line indicate log\,$U$=-2 and log(n$_{H}$/cm$^{-3}$)=3, the green solid line shows log\,$U$=-3 and log(n$_{H}$/cm$^{-3}$)=1, and the pink dashed line shows log\,$U$=-3 and log(n$_{H}$/cm$^{-3}$)=3.}
    \label{fig:miri_ar2_ar3_lmg}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{immagini/pah_6_sfg_miri_range.pdf}~
    \includegraphics[width=0.45\textwidth]{immagini/pah_7_sfg_miri_range.pdf}
    \includegraphics[width=0.45\textwidth]{immagini/s4_lmg_sfg_miri_range.pdf}
    \caption{Predicted fluxes, as a function of redshift, of a source with a total IR luminosity of L$_{IR}$=10$^{12}$L$_{\odot}$ for the 6.2$\mu$m PAH feature (a:top left); the 7.7$\mu$m PAH feature (b:top right) and for the [SIV]10.5$\mu$m line considering the SFG calibration (red solid line) and the LMG calibration (green solid line) (c:bottom). In all figures, the black solid line shows the 1 hr., 5 $\sigma$ sensitivity of JWST-MIRI, while the grey dashed line shows the 1 hr., 5 $\sigma$ sensitivity of the SPICA SMI-LR \citep{kaneda2017}.}
    \label{fig:miri_pah_s4}
\end{figure*}


Fig.\,\ref{fig:miri_ar6_mg4_ne6} shows the predicted fluxes, as a function of redshift, compared to the MIRI sensitivity for the [NeV]14.3$\mu$m (panel a), [ArVI]4.53$\mu$m (panel b), [MgIV]4.49$\mu$m (panel c) and [NeVI]7.65$\mu$m (panel d) lines, for an AGN with a total IR luminosity of L$_{IR}$=10$^{12}$L$_{\odot}$. For comparison, this figure and the following ones include also the sensitivity of the SPICA Mid-IR Instrument (SMI; grey dashed line) that was considered for the SPICA Mission \citep{roelfsema2018,spinoglio2021,kaneda2017}. This comparison indicates the better sensitivity of a cryogenically cooled space telescope at long wavelengths ($\lambda$>15$\mu$m), even of smaller diameter, such as the one of the SPICA project (2.5m), as compared to the JWST. Considering an integration time of 1~hr. and a signal to noise ratio of SNR=5, MIRI will be able to detect the [NeV] line up to redshift z$\sim$0.8. The [ArVI] line can be observed up to redshift z$\sim$1.8 for objects with an ionization parameter of $\log$U=-1.5, almost independently of the gas density, while objects with lower ionization can be observed up to redshift z$\sim$1. The [MgIV] line, instead, can be observed up to redshift z$\sim$1.8 for objects with an ionization parameter of $\log$U=-1.5, independently of the gas density. An ionization parameter of $\log$U=-2.5 expands the observational limit to z$\sim$2.8.
The [NeVI]7.65$\mu$m line can be observed up to redshift z$\sim$1.2 for objects with an ionization parameter of $\log$U=-2.5, independently of gas density. However, for a higher ionization parameter of $\log$U=-1.5 and a gas density of $\log($n$_{H}$/cm$^{-3})$=2 this line can be detected up to redshift z$\sim$1.5, and up to redshift z$\sim$1.6 if the gas density is $\log($n$_{H}$/cm$^{-3})$=4.

Fig.\,\ref{fig:miri_ar2_ar3_sf} and \ref{fig:miri_ar2_ar3_lmg} show the predicted fluxes, as a function of redshift, compared to the MIRI sensitivity, of the [NeII]12.8$\mu$m  (panel a),  [ArII]6.98$\mu$m (panel b) and [ArIII]8.99$\mu$m (panel c) lines for a SFG and a LMG of total IR luminosity of L$_{IR}$=10$^{12}$L$_{\odot}$. For the SFG, the [NeII] line can be detected up to redshift z$\sim$1 with a 1 hr. observation, while the [ArII] line can be observed up to redshift z$\sim$1.5 for models with an ionization parameter of $\log$U=-2.5, while for $\log$U=-3.5 the limiting redshift is increased to z$\sim$2.2. For the [ArIII] line, the limiting redshift is of z$\sim$1.2 independently of the adopted model.

For the LMG, the simulation yields similar results. Considering a  source of total IR luminosity of L$_{IR}$=10$^{12}$L$_{\odot}$, the [NeII] line can be detected up to z$\sim$1.25; the [ArII] line can be detected up to z$\sim$1.5 independently of the adopted model. For the [ArIII] line the maximum redshift is reached for an ionization parameter of log\,$U$=-2, and is equal to z$\sim$2, while for an ionization parameter of log\,$U$=-3 the maximum redshift is of z$\sim$1.7, independent of gas density. 

Fig.\ref{fig:miri_pah_s4} shows the predicted fluxes, as a function of redshift, compared to the MIRI sensitivity for the PAH features at 6.2 and 7.7$\mu$m (panel a and b respectively), and for the [SIV]10.5$\mu$m line considering both the SFG and LMG (panel c) calibrations for a source with total IR luminosity L$_{IR}$=10$^{12}$L$_{\odot}$. Given the high intensity of the PAH features, these can be easily detected by MIRI up to redshift z$\sim$3.6 for the 6.2$\mu$m feature, and up to redshift z$\sim$2.7 for the 7.7$\mu$m feature. The [SIV] line can instead be observed up to redshift z$\sim$1.7, but would require longer integration times to be detected in SFG  above redshift z$\sim$0.8. 

In all simulations, the decrease in sensitivity of MIRI in the 16-29$\mu$m interval raises the required exposure times to values much longer than 1 hr., in order to detect sources at higher redshift and thus probe the highly obscured galaxies at the Cosmic noon.


\subsection{Predictions for ALMA}
\label{sec:results_alma}


In this section we compare the predicted flux of the [OI]63 and 145$\mu$m, [OIII]88$\mu$m, [NII]122 and 205$\mu$m and [CII]158$\mu$m lines as a function of redshift to the sensitivity that the ALMA telescope can achieve in 1 hr. and 5 hr. observations, in order to determine the limits of the instrument in studying galaxy evolution through cosmic time. 

Fig. \ref{fig:alma_transmission} shows the atmospheric transmission at the ALMA site on Llano de Chajnantor. The transmission curve is obtained from the atmospheric radiative transfer model for ALMA by \citet{pardo2019}, and covers the 35 to 950 GHz frequency interval, equivalent to the 300$\mu$m to 3.6mm wavelength range. The figure shows the zenith atmospheric transmission for a precipitable water vapour (PWV) of 2.0mm, 1.0mm and 0.5mm. The PWV indicates the depth of water in the atmospheric column, if all the water in that column were measured as rainfall in mm. The PWV at the ALMA site is typically below 2.0mm for 65$\%$ of the year, below 1.0mm for 50$\%$ of the time and goes below 0.5mm for 25$\%$ of the time. Bands at higher frequencies (Band 9 and 10) are more affected by atmospheric transmission: considering a PWV of 1.0mm, the atmospheric transmission is $\sim$30$\%$ at 850 GHz (Band 10). Going toward shorter frequencies, the transmission goes up to $\sim$50$\%$ at 550GHz (Band 8), and $\sim$90$\%$ below 300GHz (Band 3-6). 

\begin{figure}
\centering
    \includegraphics[width=0.95\textwidth]{immagini/alma_transmission_2_1_05_pwv_2.png}
    \caption{Atmospheric transmission at the ALMA site on Llano de Chajnantor, at different frequencies, for three values of precipitable water vapour (PWV): 2.0mm (red), 1.0mm (green) and 0.5mm (blue). The vertical shaded areas show the frequency coverage of the different ALMA Bands, from AB-3 to AB-10. Figure elaborated via the on-line calculator at \url{https://almascience.nrao.edu/about-alma/atmosphere-model}. }
    \label{fig:alma_transmission}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.90\textwidth]{immagini/alma_sensitivity_o1_63.pdf}
    \includegraphics[width=0.90\textwidth]{immagini/alma_sensitivity_o3.pdf}
    
    \caption{Predicted fluxes as a fuction of redshift for the [OI]63$\mu$m line (top) and the [OIII]88$\mu$m line (bottom), compared to the ALMA sensitivity for a 1 hr. (grey dashed line) and for a 5 hrs. observation (grey dotted line) up to redshift z$\sim$9. The blue solid line shows the predicted flux using the calibration for local AGN, the red line with the calibration for local SFG, and the green solid line with the one for local LMG. The various atmospheric absorption peaks show redshift intervals that cannot be observed. The orange stars show detections for each line. }
    \label{fig:alma_sensitivity_o1_o3}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.90\textwidth]{immagini/alma_sensitivity_n2_122.pdf}
    \includegraphics[width=0.90\textwidth]{immagini/alma_sensitivity_o1_145.pdf}
    
    \caption{Predicted fluxes as a function of redshift for the [NII]122$\mu$m line (top) and the [OI]145$\mu$m line (bottom), compared to the  ALMA sensitivity for a 1 hr. (grey dashed line) and for a 5 hrs. observation (grey dotted line) up to redshift z$\sim$9. The blue solid line shows the predicted flux considering the calibration for local AGN, the red line shows the calibration for local SFG, and the green solid line shows the calibration for local LMG. The orange stars show detections for each line.}
    \label{fig:alma_sensitivity_n2_122_o1_145}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.90\textwidth]{immagini/alma_sensitivity_c2.pdf}
    \includegraphics[width=0.90\textwidth]{immagini/alma_sensitivity_n2_205.pdf}
    
    \caption{Predicted fluxes as a function of redshift for the [CII]158$\mu$m line (top) and the [NII]205$\mu$m line (bottom), compared to the ALMA sensitivity for a 1 hr. observation (grey dashed line) and for a 5 hrs. observation (grey dotted line) up to redshift z$\sim$9. The blue solid line shows the predicted flux considering the calibration for local AGN, the red line shows the calibration for local LMG. The orange stars show detections for each line.}
    \label{fig:alma_sensitivity_c2_n2_205}
\end{figure}

When determining the integration time using the ALMA sensitivity calculator\footnote{\url{https://almascience.eso.org/proposing/sensitivity-calculator}}, the PWV is automatically selected by the on-line tool to the most representative value for each band of observation.

As can be seen from Fig. \ref{fig:alma_sensitivity_o1_o3}-\ref{fig:alma_sensitivity_c2_n2_205} it has to be noticed that the ALMA sensitivity as a function of redshift is not a simple monotonic function, but contains discontinuities due to atmospheric absorption at particular frequencies. These figures show the fluxes predicted for various lines as a function of redshift for a source of total IR luminosity of L$_{IR}$=10$^{12.5}$L$_{\odot}$, compared to the ALMA sensitivity in 1 hr. and 5 hrs. reaching a signal-to-noise $\sigma$=5, assuming the line calibrations for SFG, LMG and AGN presented in \citet{mordini2021}.
We have chosen the luminosity of L$_{IR}$=10$^{12.5}$L$_{\odot}$ because it corresponds to the luminosity of a MS galaxy of mass of M$_{\star}$=10$^{10.7}$ M$_{\odot}$ at a redshift z=4 \citep{scoville2017}.

In Fig.\,\ref{fig:alma_sensitivity_o1_o3} we show the fluxes predicted for the [OI]63$\mu$m (top) and [OIII]88$\mu$m (bottom) lines as a function of redshift. 
The [OI]63$\mu$m line could in principle be observed by ALMA starting from the redshift of z$\sim$4 and up to a redshift of z$\sim$8. However, the line is observable only using ALMA bands 9 and 10, making it rather difficult to detect, due to the low atmospheric transmission. Considering the LMG calibration, the line would require an integration time of $\sim$5 hrs. to be detected, while for the SFG and AGN calibrations the observational time would be between 10 and 20 hrs. This value is unrealistic for a ground-based telescope, such as ALMA, and in principle could be achieved only by summing up the results of various observing runs of few hours each. As a matter of fact, the only detection of the [OI]63$\mu$m line available so far for a high-redshift galaxy is the one reported by \citet{rybak2020} for a strongly gravitationally lensed galaxy (magnification $\mu_{FIR}\simeq$9) obtained with the APEX 12m telescope \citep{gusten2006}, and the Swedish ESO PI (SEPIA) Band 9 receiver \citep{belitsky2018}, shown in the figure. The [OIII]88$\mu$m line, on the other hand, can be observed from redshift z$\sim$3. For this line, galaxies that present physical characteristics similar to local LMG can be easily detected with observations shorter than 1 hr., while for SFG and AGN, observational times longer than 5 hrs. are required up to redshift z$\sim$8. In the figure, we report [OIII]88$\mu$m detections by \citet{vishwas2018,walter2018,debreuck2019,tamura2019,harikane2019}. We note that, while all reported detections have $\sigma$=5 or higher, the integration times can reach values of the order of 7.5hrs. Moreover, we do not correct the line luminosities for the magnification effect, when present.

In Fig.\,\ref{fig:alma_sensitivity_n2_122_o1_145} we show the fluxes predicted for the [NII]122$\mu$m (top) and [OI]145$\mu$m (bottom) lines as a function of redshift.
In AGN, the [NII] line can be detected with an integration time of less than 1 hr., from a redshift of z$\sim$1.8. For SFG, the line can be detected with observations of the order of 5 hrs. only for redshifts above z$\sim$6, while at lower redshifts, or for  LMG, the observational times needed to detect this line are larger than 5 hrs. The [OI]145$\mu$m line  can be observed with integration times of the order of 5hr. above redshift z$\sim$4 in SFG and LMG, while in AGN or for lower redshifts longer integration times are needed. In the figure we also report a detection for [NII]122$\mu$m and [OI]145$\mu$m \citep{debreuck2019}.

Finally, Fig.\,\ref{fig:alma_sensitivity_c2_n2_205} shows the predicted fluxes for the [CII]158 $\mu$m (top) and the [NII]205$\mu$m (bottom) lines. The [CII] line is by far the brightest far-IR fine-structure line in galaxies and given its longer wavelength it can be detected in the redshift ranges of 0.9$\lesssim$z$\lesssim$2 and 3$\lesssim$z$\lesssim$9, requiring integration times shorter than 1 hr. independently of the galaxy type. The [NII]205$\mu$m line can be detected from redshift z$\sim$0.5, however it requires at least 1 hr. of observation up to z$\sim$3, and a longer integration at higher redshifts for SFG. For AGN the line appears weaker, and requires integration times longer than 5 hrs. to be detected. We include the detections for the [CII]158$\mu$m line reported by \citet{faisst2020,venemans2020} and for the [NII]205$\mu$m line by \citet{cunningham2020}, considering only objects with $\sigma$=5 or higher.

While in our calculations we have considered a source with a total IR luminosity of L$_{IR}$=10$^{12.5}$L$_{\odot}$, brighter galaxies, or sources whose apparent flux is enhanced by gravitational lensing, can be detected in shorter integration times.


\section{DISCUSSION}
\label{sec:discussion}
\begin{figure*}
    \centering
    \includegraphics[width=0.456\textwidth]{immagini/sfr_miri.png}
    \includegraphics[width=0.44\textwidth]{immagini/bhar_miri.png}
    \caption{ ({\bf a: left}) Star formation rate (SFR, in M$_{\odot}$\,yr$^{-1}$) as a function of redshift for a 10$^{10.7}$ M$_{\odot}$ galaxy in the Main Sequence \citep[MS,][]{scoville2017} as a red solid line.
    The redddish shaded area shows the 0.35 dex intrinsic scatter around the MS \citep{schreiber2015} and the dark and light orange shaded areas indicate the  +2$\sigma$ and +3$\sigma$ lines above the MS, respectively. The observability limits for the lines are shown as: black dash-dotted line: [ArIII]8.99$\mu$m for a SFG with t$_{INT}$ =1hr; blue dashed line: same line for a LMG (in both cases the highest line ratio present in Table \ref{tab:line_ratios} was adopted);  pink dotted line: the PAH feature at 6.2$\mu$m; green solid line: the PAH feature at 7.7$\mu$m. In these latter cases, we derived the limit from the correlations in \citet{mordini2021}.\\
    ({\bf b: right}) The green solid line indicates the instantaneous BH accretion rate (BHAR, in M$_{\odot}$\,yr$^{-1}$) as a function of redshift expected for a MS galaxy with a mass of 10$^{10.7}$ M$_{\odot}$ during its active BH accretion phase at each epoch, using the SFR-BHAR relation of \citet{diamondstanic2012}. The green shaded area shows the associated dispersion. The observability limits for the lines are shown as: purple dotted line: the [NeVI]7.65$\mu$m line; blue dashed line: the [ArVI]4.53$\mu$m; red solid line: the [MgIV]4.49$\mu$m line. 
    For all three lines, we considered a 1hr. pointed observation, and the highest line ratio as reported in Table \ref{tab:line_ratios}. In both panels, the grey hatched areas indicate the parameter space that requires observations longer than 1hr.}
    \label{fig:sfr_bhar_miri}
\end{figure*}

We derive here the predictions to measure the BHAR and SFR with the JWST-MIRI spectrometer, following the same method that has been prepared for the scientific assessment of the galaxy evolution observational program \citep{spinoglio2021} for the SPICA mission \citep{roelfsema2018}. In this study, the predictions of measuring the SFR and the BHAR with the 2.5m SPICA telescope have been carried out using the [NeII]12.8$\mu$m and [NeIII]15.5$\mu$m lines for the SFR and [OIV]26$\mu$m for the BHAR \citep[see Fig. 9 of ][]{spinoglio2021}, while for JWST-MIRI we use shorter wavelength lines.

Fig.\ref{fig:sfr_bhar_miri}(a) shows the SFR of a galaxy in the Main Sequence \citep[MS; ][]{rodighiero2010,elbaz2011}, with values of luminosities as a function of redshift taken from \citet{scoville2007}, assuming a galaxy with a stellar mass of M$_{\star}$=10$^{10.7}$ M$_{\odot}$ \citep{muzzin2013,adams2021} and an associated dispersion around the MS of 0.35 dex \citep[red shaded area; ][]{schreiber2015}. The relation between luminosity and SFR has been taken from \citet{kennicutt2012}. The various colored lines indicate the JWST-MIRI sensitivity limit for a 1 hr. pointed observation, considering the PAH features at 6.2 and 7.7$\mu$m for SFG and the [ArIII]8.99$\mu$m line for both SFG and LMG, as discussed in Section \ref{sec:results_jwst}. For the PAH features, we considered the line calibrations reported in \citet{mordini2021}, while for the fine structure lines we considered the best case scenario, thus selecting the highest possible line ratio reported in Table \ref{tab:line_ratios}, and thus the physical conditions yielding the brightest lines. The PAH features at 6.2$\mu$m and 7.7$\mu$m are the best tracers for the SFR, covering the population below the MS up to redshift z$\sim$3, which equals a minimum luminosity between L$_{IR}\sim$10$^{9.5}$M$_{\odot}$ observable at z$\sim$1 and L$_{IR}\sim$10$^{12.5}$M$_{\odot}$ observable at z$\sim$3. The [ArIII]8.99$\mu$m line, on the other hand, can be detected in MS galaxies up to redshift z$\sim$1.8 (observable luminosities between L$_{IR}\sim$10$^{11}$M$_{\odot}$ at z$\sim$1 and L$_{IR}\sim$10$^{13}$M$_{\odot}$ at z$\sim$2.2). This poses a limit to the study of LMG at higher redshifts, since the reduced formation efficiency and the increased stellar radiation hardness reduces the strength of the PAH features in these objects, which are only detected at metallicities above 1/8-1/10 Z$_{\odot}$ \citep{engelbracht2008,cormier2015,galliano2021}. 

The results presented for the ALMA telescope suggest that the [CII]158$\mu$m line, a proxy for measuring SFR, can be easily observed in objects at redshift z$\gtrsim$3, thus allowing to trace the evolution of SFR throughout cosmic time. At the present time, this line has been observed by ALMA in the z$\sim$4-7 redshift interval \citep[see e.g. ][]{hashimoto2019,faisst2020}. An alternative can be offered by the sum of the [OIII]88$\mu$m and [OI]145$\mu$m lines, in analogy to the [OI]63$\mu$m plus [OIII]88$\mu$m tracer proposed in \citet{mordini2021}: the [OI]145$\mu$m can be detected with ALMA from redshift z$\sim$1.5 with observations of $\sim$5\,hr for SFG and LMG-like sources, and, unlike the [OI]63$\mu$m line, is not affected by self-absorpion. 

We report, from \citet{mordini2021}, the correlation between the SFR and the PAH 6.2$\mu$m feature luminosity (equation \ref{eq:pah_sfr}), and between the SFR and the [CII]158$|mu$m line luminosity (equation \ref{eq:c2_sfr}):

\begin{multline}\label{eq:pah_sfr}
    \log\left(\frac{SFR}{\rm M_{\odot}\,yr^{-1}}\right)=(0.37 \pm 0.04)\\+(0.76 \pm 0.03)\log\left(\frac{L_{PAH6.2}}{\rm 10^{41}\,erg\,s^{-1}}\right)
\end{multline}

\begin{multline}\label{eq:c2_sfr}
\log\left ( \frac{SFR}{\rm M_{\odot}\,yr^{-1}}\right )=(0.62 \pm 0.02)\\ +(0.89 \pm 0.02) \left( \log\frac{L_{[CII]}}{\rm 10^{41}\,erg\,s^{-1}}\right )
\end{multline}

with the line luminosities espressed in units of 10$^{41}$\,erg\,s$^{-1}$, and the SFR in M$_{\odot}$\,yr$^{-1}$. We also derive a possible correlation between the SFR and the sum of the [ArII]7.0$\mu$m and [ArIII]9.0$\mu$m lines, considering the [NeII]12.8$\mu$m plus [NeIII]15.6$\mu$m SFR tracer \citep[see Section 3.2.4 in ][ for details]{mordini2021}, and the ([ArII]+[ArIII])/([NeII]+[NeIII]) ratio (reported in Table \ref{tab:line_ratios}). This leads to a SFR to ([ArII]+[ArIII]) lines luminosity correlation for SFG reported in equation \ref{eq:ar2_ar3_sfr_sfg}, while equation \ref{eq:ar2_ar3_sfr_lmg} reports the same correlation for LMG:



\begin{multline}\label{eq:ar2_ar3_sfr_sfg}
 \log\left(\frac{SFR}{\rm M_{\odot}\,yr^{-1}}\right)= 1.28\\ +0.96 \log\left( \frac{L_{\rm [ArII]+[ArIII]}}{\rm 10^{41}\,erg\,s^{-1}}\right),
\end{multline}

\begin{multline}\label{eq:ar2_ar3_sfr_lmg}
 \log\left(\frac{SFR}{\rm M_{\odot}\,yr^{-1}}\right)= 1.57\\ +0.96 \log\left( \frac{L_{\rm [ArII]+[ArIII]}}{\rm 10^{41}\,erg\,s^{-1}}\right).
\end{multline}

\begin{figure}
    \centering
    \includegraphics[width=0.85\columnwidth]{immagini/o3_sfr_sf_dwarf.pdf}
    \caption{Correlation between the [OIII]88$\mu$m and [OI]145$\mu$m summed emission line luminosities, in units of $10^{41}\, \rm{erg\,s^{-1}}$, and the SFR derived from the total IR luminosity (black dashed line) for a composite sample of SFGs (red stars) and from the H$_{\alpha}$ luminosity (corrected for the IR luminosity) for LMG (green triangles). We remand the reader to Section 3 in \citet{mordini2021} for details on the determination of the SFR.}
    \label{fig:o1_o3_sfr}
\end{figure}


Lastly we determined, for local galaxies, a correlation between the SFR [OIII]88$\mu$m plus [OI]145$\mu$m lines. Fig.\,\ref{fig:o1_o3_sfr} shows the correlation described by the equation:

\begin{multline}
 \log\left(\frac{SFR}{\rm M_{\odot}\,yr^{-1}}\right)= (0.52 \pm 0.14)\\ +(0.93 \pm 0.14) \log\left( \frac{L_{\rm [OI]+[OIII]}}{\rm 10^{41}\,erg\,s^{-1}}\right).
\end{multline}

The correlation was obtained using 23 local galaxies, of which 11 SFG \citep[from ][]{negishi2015} and 12 LMG \citep[from ]{cormier2015}, and has a Pearson $r$ coefficient of 0.77. The low number of objects used to derive this correlation is due to a low number of detections of the [OI]145$\mu$m line in local galaxies, which broadens the confidence interval of the relation, reported in Fig.\,\ref{fig:o1_o3_sfr} as a shaded area.


Fig.\ref{fig:sfr_bhar_miri}(b) shows instead the instantaneous BHAR as a function of redshift for an AGN in a MS star-forming galaxy with M$^{*}$=10$^{10.7}$ M$_{\odot}$, using the SFR-BHAR calibration derived by \citet{diamondstanic2012} for a sample of nearby Seyfert galaxies. The green shaded area corresponds to the dispersion of the SFR-BHAR relation, i.e. $\sim$ 0.9 dex. This estimate, however, considers only the portion of galaxies in the MS undergoing a BH accreting phase at each epoch, with the instantaneous BHAR that has not been averaged over the duty cycle of the active nucleus. The dashed lines represent the three proposed tracers for BHAR in Section \ref{sec:results_jwst}, considering a 1 hr. pointed observation: the [MgIV]4.49$\mu$m line appears to be the best tracer for BHAR, reaching galaxies below the main sequence up to redshift z$\sim$2.5 (observable luminosities between L$_{IR}\sim$10$^{10.5}$M$_{\odot}$ at z$\sim$1 and L$_{IR}\sim$10$^{12.5}$M$_{\odot}$ at z$\sim$4). The possibility of detecting the [ArVI] and [NeVI] lines only in bright galaxies is due to the higher ionization potential needed to excite these lines (respectively of 80\,eV and 126\,eV, see Table \ref{tab:line_properties}). It is important to consider that these lines have not been extensively observed yet, and these predictions are based on CLOUDY photo-ionization models. Considering the line ratios reported in Table \ref{tab:line_ratios} and the BHAR-[NeV]14.3 correlation derived in \citet{mordini2021}, we attempt to derive a possible correlation between the BHAR and the [MgIV]4.5$\mu$m line (reported in equation \ref{eq:mg4_bhar}), and between the BHAR and the [ArVI]4.5$\mu$m line (reported in equation \ref{eq:ar6_bhar}):

\begin{equation}\label{eq:lusso_ne5_14}
    \log\left(\frac{\dot{M}_{BH}}{\rm M_{\odot}\,yr^{-1}}\right)=-0.85+1.04\log\left(\frac {L_{\rm [MgIV]4.5}}{\rm 10^{41}\,erg\,s^{-1}}\right)
\end{equation}

\begin{equation}\label{eq:lusso_ne5_14}
\log\left(\frac{\dot{M}_{BH}}{\rm M_{\odot}\,yr^{-1}}\right)=0.58+1.04\log\left(\frac {L_{\rm [ArVI]4.5}}{\rm 10^{41}\,erg\,s^{-1}}\right)
\end{equation}

The hatched areas in both panels of Fig.\ref{fig:sfr_bhar_miri} indicate the region where observations longer than 1 hr are required. A longer exposure time can significantly improve these limits, allowing the JWST-MIRI spectrometer to study both SFR and BHAR in MS galaxies up to redshift z$\sim$3. 

Among the far-IR lines covered by the ALMA telescope at redshifts higher than z$\sim$3, the only available tracers for BH activity are represented by the [OIII]52 and 88$\mu$m lines. Their ionization potential ($\sim$35\,eV, see Table \ref{tab:line_properties}) is sufficiently high to be excited by AGN. However, these lines are also associated to stellar and HII regions excitation, thus limiting their potential as BHA tracer. A set of observed far-IR lines or the specific photo-ionization models that could simulate the two emission components \citep[see, e.g.][]{spinoglio1995} are needed to disentangle the stellar emission from the total observed emission of these lines.



The inability of performing wide area surveys (of the order of square degrees) with either facility, however, imposes a significant limit to the possibility of characterizing galaxy evolution: while the tracers proposed in this work can be used to trace both star formation and BHA at the Cosmic Noon, a complete study of galaxy evolution also requires to account for the environment within which galaxies evolve, thus incorporating the large scale structure of the Universe, by mapping large cosmological volumes. Moreover, even using both facilities together, it is not possible to perform accurate analysis on galaxy evolution covering both the cosmic noon and the higher redshifts. On the one hand, in fact, while the PAH features can be detected with JWST up to redshift z$\sim$2.5 in MS galaxies, and at higher redshifts the ALMA telescope can trace star formation activity with the [CII]158$\mu$m line, there is the problem of tracing SF in low metallicity environments, where the PAH features are weak or absent, or in high luminosity galaxies, where the [CII] deficit can lead to lower determinations of the SFR \citep[see e.g. ][]{ferrara2019}. On the other hand, ALMA lacks an unambiguous tracer for BHA activity, and the proposed tracers for JWST only reach redshift z$\sim$3 for MS galaxies.

A full characterization of the obscured phase of galaxy evolution at the cosmic noon will have to wait for a new IR space telescope, actively cooled down to a few degrees Kelvin and with state of the art detectors, able to perform wide area spectroscopic surveys covering most of the mid- to far-IR range (i.e. between 10$\mu$m and 300$\mu$m). Possible candidate missions include the very ambitious \emph{Origins Space Telescope} \citep[OST, ][]{meixner2019} and the smaller size \emph{Galaxy Evolution Probe} telescope \citep[GEP, ][]{glenn2021}, which has the main goal to map the history of galaxy growth through star formation and accretion by supermassive black holes and to characterize the relationship between these two processes. The pioneering study of the scientific potential of an IR space telescope for galaxy evolution studies throughout cosmic time has been provided by \citet{spinoglio2017, spinoglio2021}, based on the SPICA mission project \citep{swinyard2009, roelfsema2018}.


\section{CONCLUSIONS}
\label{sec:conclusions}

In this work we present spectroscopic tracers for star formation and BHA activity that can be used by the JWST and the ALMA telescopes to characterize galaxy evolution up to and beyond the Cosmic Noon, respectively. In particular, our findings can be summarized as follow:

\begin{itemize}
\item The JWST-MIRI instrument in spectroscopic mode will be able to detect mid-IR spectra of faint fine-structure lines and PAH features in galaxies at redshift z$\gtrsim$1 and discriminate between AGN-dominated and starburst-dominated galaxies and measure their metallicity.

\item The presence of an AGN can be detected using high ionization lines such as the [ArVI]4.5$\mu$m, [MgIV]4.49$\mu$m or [NeVI]7.65$\mu$m lines: the [ArVI] and [MgIV] lines can be observed up to redshift z$\sim$3, while the [NeVI] line can be observed up to redshift z$\sim$1.5 in a 1hr observation.

\item For the star formation processes using JWST, the PAH features can be easily detected up to redshift z$\sim$2.7, while the [ArII]6.98$\mu$m and [ArIII]8.99$\mu$m lines can be detected up to redshift z$\sim$2.5-3. The detection of the [SIV]10.5$\mu$m line can discriminate between solar and sub-solar metallicity: in LMG, the [SIV] line can be easily detected up to redshift z$\sim$1.5, while in solar metallicity SFG, this line is so weak that cannot be detected above redshift z$\sim$0.8.

\item Using the ALMA observatory, the far-IR oxygen lines of  [OIII]88$\mu$m and [OI]145$\mu$m can be detected (with integration times of 1 to 5 hrs.) preferentially in galaxies characterized by a low metallicity (LMG). In AGN or normal SFG, the [OIII]88$\mu$m line needs t$_{INT}$ $\gtrsim$ 5 hrs.
Due to the high observing frequency, where the sky transparency is very low,  the [OI]63$\mu$m can hardly be detected in t$_{INT}$ $\gtrsim$ 5 hrs. and only if the galaxy is an LMG. 
On the contrary the [NII]122$\mu$m line is preferentially detected in AGN and normal star forming galaxies (SFG). The [NII]205$\mu$m can hardly be detected with t$_{INT}$ $\gtrsim$ 5 hrs in AGN and SFG. 

\item The [CII]158$\mu$m line can be easily detected in any galaxy type at redshift of 0.9$\lesssim$z$\lesssim$2 and 3$\lesssim$z$\lesssim$9.
It remains the best tracers for SFG and can measure their SFR, but can also be easily detected in AGN. Among other SFR tracers, in analogy with the proposed  [OI]63$\mu$m plus [OIII]88$\mu$m tracer analyzed in \citet{mordini2021}, we suggest the use of the [OIII]88$\mu$m plus [OI]145$\mu$m for high redshift sources.  The [OI]145$\mu$m can be detected with ALMA starting from redshift z$\sim$1.5 with observations of $\sim$5\,hr for SFG and LMG-like sources. While in local SFG and LMG there are not enough detections of the [OI]145$\mu$m line to appropriately test it as SFR tracer, this line, although fainter,  should be even better than the  [OI]63$\mu$m, which can be strongly self-absorbed under certain conditions \citep[see, e.g.,][]{liseau2006} and should allow to measure the SFR in combination with the [OIII]88$\mu$m line.

\end{itemize}


\begin{acknowledgement}
LS and JAFO acknowledge financial support by the Agenzia Spaziale Italiana (ASI) under the research contract 2018-31-HH.0. JAFO acknowledges the financial support from the European Union - NextGenerationEU and the Spanish Ministry of Science and Innovation through the Recovery and Resilience Facility project J-CAVA.
\end{acknowledgement}
